Improved generalization with deep neural operators for engineering systems: Path towards digital twin

Neural Operator Networks (ONets) represent a novel advancement in machine learning algorithms, offering a robust and generalizable alternative for approximating partial differential equations (PDEs) solutions. Unlike traditional Neural Networks (NN), which directly approximate functions, ONets specialize in approximating mathematical operators, enhancing their efficacy in addressing complex PDEs. In this work, we evaluate the capabilities of Deep Operator Networks (DeepONets), an ONets implementation using a branch/trunk architecture. Three test cases are studied: a system of ODEs, a general diffusion system, and the convection/diffusion Burgers equation. It is demonstrated that DeepONets can accurately learn the solution operators, achieving prediction accuracy scores above 0.96 for the ODE and diffusion problems over the observed domain while achieving zero shot (without retraining) capability. More importantly, when evaluated on unseen scenarios (zero shot feature), the trained models exhibit excellent generalization ability. This underscores ONets vital niche for surrogate modeling and digital twin development across physical systems. While convection-diffusion poses a greater challenge, the results confirm the promise of ONets and motivate further enhancements to the DeepONet algorithm. This work represents an important step towards unlocking the potential of digital twins through robust and generalizable surrogates.

==> 1 <==
\begin{thebibliography}{49}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Lu et~al.(2021{\natexlab{a}})Lu, Jin, Pang, Zhang, and
  Karniadakis]{DeepONet_Lu}
Lu~Lu, Pengzhan Jin, Guofei Pang, Zhongqiang Zhang, and George~Em Karniadakis.
\newblock Learning nonlinear operators via deeponet based on the universal
  approximation theorem of operators.
\newblock \emph{Nature Machine Intelligence 2021 3:3}, 3:\penalty0 218--229, 3
  2021{\natexlab{a}}.
\newblock ISSN 2522-5839.
\newblock \doi{10.1038/s42256-021-00302-5}.
\newblock URL \url{https://www.nature.com/articles/s42256-021-00302-5}.

\bibitem[Kovachki et~al.(2021)Kovachki, Li, Edu, Liu, Azizzadenesheli,
  Bhattacharya, Stuart, and Anandkumar]{operator_maps_kovachki}
Nikola Kovachki, Zongyi Li, Zongyili@caltech Edu, Caltech~Burigede Liu, Kamyar
  Azizzadenesheli, Kaushik Bhattacharya, Andrew Stuart, and Anima Anandkumar.
\newblock Neural operator: Learning maps between function spaces.
\newblock 8 2021.
\newblock \doi{10.48550/arxiv.2108.08481}.
\newblock URL \url{https://arxiv.org/abs/2108.08481v4}.

\bibitem[Wang et~al.(2022)Wang, Wang, and
  Perdikaris]{architectures_algorithms_wang}
Sifan Wang, Hanwen Wang, and Paris Perdikaris.
\newblock Improved architectures and training algorithms for deep operator
  networks.
\newblock \emph{Journal of Scientific Computing}, 92:\penalty0 1--42, 8 2022.
\newblock ISSN 15737691.
\newblock \doi{10.1007/S10915-022-01881-0/FIGURES/27}.
\newblock URL
  \url{https://link.springer.com/article/10.1007/s10915-022-01881-0}.

\bibitem[Li et~al.(2022{\natexlab{a}})Li, Huang, Liu, and
  Anandkumar]{fourier_pde_li}
Zongyi Li, Daniel~Zhengyu Huang, Burigede Liu, and Anima Anandkumar.
\newblock Fourier neural operator with learned deformations for pdes on general
  geometries.
\newblock 7 2022{\natexlab{a}}.
\newblock \doi{10.48550/arxiv.2207.05209}.
\newblock URL \url{https://arxiv.org/abs/2207.05209v1}.

\bibitem[Lu et~al.(2022{\natexlab{a}})Lu, Pestourie, Johnson, and
  Romano]{deeponet_heat_lu}
Lu~Lu, Raphaël Pestourie, Steven~G. Johnson, and Giuseppe Romano.
\newblock Multifidelity deep neural operators for efficient learning of partial
  differential equations with application to fast inverse design of nanoscale
  heat transport.
\newblock \emph{Physical Review Research}, 4, 4 2022{\natexlab{a}}.
\newblock ISSN 26431564.
\newblock \doi{10.48550/arxiv.2204.06684}.
\newblock URL \url{https://arxiv.org/abs/2204.06684v1}.

\bibitem[Garg et~al.(2022{\natexlab{a}})Garg, Gupta, and
  Chakraborty]{deeponet_stochastic_souvik}
Shailesh Garg, Harshit Gupta, and Souvik Chakraborty.
\newblock Assessment of deeponet for reliability analysis of stochastic
  nonlinear dynamical systems.
\newblock 1 2022{\natexlab{a}}.
\newblock \doi{10.48550/arxiv.2201.13145}.
\newblock URL \url{https://arxiv.org/abs/2201.13145v1}.

\bibitem[Yu et~al.(2002)Yu, Efe, and Kaynak]{nn_backpropagation_yu}
Xinghuo Yu, M.~Onder Efe, and Okyay Kaynak.
\newblock A general backpropagation algorithm for feedforward neural networks
  learning.
\newblock \emph{IEEE Transactions on Neural Networks}, 13:\penalty0 251--254, 1
  2002.
\newblock ISSN 10459227.
\newblock \doi{10.1109/72.977323}.

\bibitem[Schmidhuber(2015)]{deep_learning_overview_schmidhuber}
Jürgen Schmidhuber.
\newblock Deep learning in neural networks: An overview.
\newblock \emph{Neural Networks}, 61:\penalty0 85--117, 1 2015.
\newblock ISSN 0893-6080.
\newblock \doi{10.1016/J.NEUNET.2014.09.003}.

\bibitem[Anastassiou(2011)]{tanh_approx_anastassiou}
George~A. Anastassiou.
\newblock Multivariate hyperbolic tangent neural network approximation.
\newblock \emph{Computers \& Mathematics with Applications}, 61:\penalty0
  809--821, 2 2011.
\newblock ISSN 0898-1221.
\newblock \doi{10.1016/J.CAMWA.2010.12.029}.

\bibitem[Cardaliaguet and Euvrard(1992)]{nn_approx_cardaliaguet}
Pierre Cardaliaguet and Guillaume Euvrard.
\newblock Approximation of a function and its derivative with a neural network.
\newblock \emph{Neural Networks}, 5:\penalty0 207--220, 1 1992.
\newblock ISSN 0893-6080.
\newblock \doi{10.1016/S0893-6080(05)80020-6}.

\bibitem[Selmic and Lewis(2002)]{nn_piecewise_selmic}
Rastko~R. Selmic and Frank~L. Lewis.
\newblock Neural-network approximation of piecewise continuous functions:
  Application to friction compensation.
\newblock \emph{IEEE Transactions on Neural Networks}, 13:\penalty0 745--751, 5
  2002.
\newblock ISSN 10459227.
\newblock \doi{10.1109/TNN.2002.1000141}.

\bibitem[Li et~al.(2020)Li, Kovachki, Azizzadenesheli, Liu, Bhattacharya,
  Stuart, and Anandkumar]{fourier_operator_kovachki}
Zongyi Li, Nikola Kovachki, Kamyar Azizzadenesheli, Burigede Liu, Kaushik
  Bhattacharya, Andrew Stuart, and Anima Anandkumar.
\newblock Fourier neural operator for parametric partial differential
  equations.
\newblock 10 2020.
\newblock \doi{10.48550/arxiv.2010.08895}.
\newblock URL \url{https://arxiv.org/abs/2010.08895v3}.

\bibitem[Marcati and Schwab(2021)]{onet_elliptic_eq_marcati}
Carlo Marcati and Christoph Schwab.
\newblock Exponential convergence of deep operator networks for elliptic
  partial differential equations.
\newblock 12 2021.
\newblock \doi{10.48550/arxiv.2112.08125}.
\newblock URL \url{https://arxiv.org/abs/2112.08125v2}.

\bibitem[Zhu et~al.(2022)Zhu, Zhang, Jiao, Karniadakis, and Lu]{sparse_obs_zhu}
Min Zhu, Handi Zhang, Anran Jiao, George~Em Karniadakis, and Lu~Lu.
\newblock Reliable extrapolation of deep neural operators informed by physics
  or sparse observations.
\newblock 12 2022.
\newblock \doi{10.48550/arxiv.2212.06347}.
\newblock URL \url{https://arxiv.org/abs/2212.06347v1}.

\bibitem[de~Hoop et~al.(2022)de~Hoop, Huang, null, and
  Stuart]{cost_accuracy_hoop}
Maarten~V. de~Hoop, Daniel~Zhengyu Huang, Elizabeth~Qian null, and Andrew~M.
  Stuart.
\newblock The cost-accuracy trade-off in operator learning with neural
  networks.
\newblock \emph{Journal of Machine Learning}, 1:\penalty0 299--341, 3 2022.
\newblock ISSN 2790-203X.
\newblock \doi{10.48550/arxiv.2203.13181}.
\newblock URL \url{https://arxiv.org/abs/2203.13181v3}.

\bibitem[Yin et~al.(2022)Yin, Zhang, Yu, and Karniadakis]{fem_operator_yin}
Minglang Yin, Enrui Zhang, Yue Yu, and George~Em Karniadakis.
\newblock Interfacing finite elements with deep neural operators for fast
  multiscale modeling of mechanics problems.
\newblock \emph{Computer Methods in Applied Mechanics and Engineering},
  402:\penalty0 115027, 12 2022.
\newblock ISSN 0045-7825.
\newblock \doi{10.1016/J.CMA.2022.115027}.

\bibitem[Lin et~al.(2021{\natexlab{a}})Lin, Li, Lu, Cai, Maxey, and
  Karniadakis]{bubble_growth_lin}
Chensen Lin, Zhen Li, Lu~Lu, Shengze Cai, Martin Maxey, and George~Em
  Karniadakis.
\newblock Operator learning for predicting multiscale bubble growth dynamics.
\newblock \emph{The Journal of Chemical Physics}, 154:\penalty0 104118, 3
  2021{\natexlab{a}}.
\newblock ISSN 0021-9606.
\newblock \doi{10.1063/5.0041203}.
\newblock URL \url{https://aip.scitation.org/doi/abs/10.1063/5.0041203}.

\bibitem[Lin et~al.(2021{\natexlab{b}})Lin, Maxey, Li, and
  Karniadakis]{bubble_dynamics_lin}
Chensen Lin, Martin Maxey, Zhen Li, and George~Em Karniadakis.
\newblock A seamless multiscale operator neural network for inferring bubble
  dynamics.
\newblock \emph{Journal of Fluid Mechanics}, 929:\penalty0 A18, 12
  2021{\natexlab{b}}.
\newblock ISSN 0022-1120.
\newblock \doi{10.1017/JFM.2021.866}.
\newblock URL
  \url{https://www.cambridge.org/core/journals/journal-of-fluid-mechanics/article/abs/seamless-multiscale-operator-neural-network-for-inferring-bubble-dynamics/D516AB0EF954D0FF56AD864DB2618E94}.

\bibitem[Pickering and Sapsis(2022)]{operator_uncertainty_pickering}
Ethan Pickering and Themistoklis~P. Sapsis.
\newblock Structure and distribution metric for quantifying the quality of
  uncertainty: Assessing gaussian processes, deep neural nets, and deep neural
  operators for regression.
\newblock 3 2022.
\newblock \doi{10.48550/arxiv.2203.04515}.
\newblock URL \url{https://arxiv.org/abs/2203.04515v1}.

\bibitem[Tripura and Chakraborty(2022)]{wavelet_parametric_pde_souvik}
Tapas Tripura and Souvik Chakraborty.
\newblock Wavelet neural operator: a neural operator for parametric partial
  differential equations.
\newblock 5 2022.
\newblock ISSN 00457825.
\newblock \doi{10.48550/arxiv.2205.02191}.
\newblock URL \url{https://arxiv.org/abs/2205.02191v1}.

\bibitem[Lu et~al.(2022{\natexlab{b}})Lu, Meng, Cai, Mao, Goswami, Zhang, and
  Karniadakis]{operator_comparison_lu}
Lu~Lu, Xuhui Meng, Shengze Cai, Zhiping Mao, Somdatta Goswami, Zhongqiang
  Zhang, and George~Em Karniadakis.
\newblock A comprehensive and fair comparison of two neural operators (with
  practical extensions) based on fair data.
\newblock \emph{Computer Methods in Applied Mechanics and Engineering},
  393:\penalty0 114778, 4 2022{\natexlab{b}}.
\newblock ISSN 0045-7825.
\newblock \doi{10.1016/J.CMA.2022.114778}.

\bibitem[Gorban and Wunsch(2002)]{Gorban2002}
A.N. Gorban and D.C. Wunsch.
\newblock The general approximation theorem.
\newblock pages 1271--1274, 11 2002.
\newblock \doi{10.1109/IJCNN.1998.685957}.

\bibitem[Chen and Chen(1995)]{Chen1995}
Tianping Chen and Hong Chen.
\newblock Universal approximation to nonlinear operators by neural networks
  with arbitrary activation functions and its application to dynamical systems.
\newblock \emph{IEEE Transactions on Neural Networks}, 6:\penalty0 911--917,
  1995.
\newblock ISSN 19410093.
\newblock \doi{10.1109/72.392253}.

\bibitem[Goswami et~al.(2022)Goswami, Bora, Yu, and Karniadakis]{pino_goswami}
Somdatta Goswami, Aniruddha Bora, Yue Yu, and George~Em Karniadakis.
\newblock Physics-informed deep neural operator networks.
\newblock 7 2022.
\newblock \doi{10.48550/arxiv.2207.05748}.
\newblock URL \url{https://arxiv.org/abs/2207.05748v2}.

\bibitem[Guan et~al.(2021)Guan, Hsu, and Guan]{fno_acoustic_guan}
Steven Guan, Ko-Tsung Hsu, and Parag V Chitnis~S Guan.
\newblock Fourier neural operator networks: A fast and general solver for the
  photoacoustic wave equation.
\newblock page 22102, 8 2021.
\newblock \doi{10.48550/arxiv.2108.09374}.
\newblock URL \url{https://arxiv.org/abs/2108.09374v1}.

\bibitem[Thakur et~al.(2022)Thakur, Tripura, and
  Chakraborty]{multifidelity_wavelet_souvik}
Akshay Thakur, Tapas Tripura, and Souvik Chakraborty.
\newblock Multi-fidelity wavelet neural operator with application to
  uncertainty quantification.
\newblock 8 2022.
\newblock \doi{10.48550/arxiv.2208.05606}.
\newblock URL \url{https://arxiv.org/abs/2208.05606v1}.

\bibitem[Pickering et~al.(2022)Pickering, Guth, Karniadakis, and
  Sapsis]{extreme_forecasting_pickering}
Ethan Pickering, Stephen Guth, George~Em Karniadakis, and Themistoklis~P.
  Sapsis.
\newblock Discovering and forecasting extreme events via active learning in
  neural operators.
\newblock \emph{Nature Computational Science 2022 2:12}, 2:\penalty0 823--833,
  12 2022.
\newblock ISSN 2662-8457.
\newblock \doi{10.1038/s43588-022-00376-0}.
\newblock URL \url{https://www.nature.com/articles/s43588-022-00376-0}.

\bibitem[Lu et~al.(2021{\natexlab{b}})Lu, Meng, Mao, and
  Karniadakis]{lu2021deepxde}
Lu~Lu, Xuhui Meng, Zhiping Mao, and George~Em Karniadakis.
\newblock {DeepXDE}: A deep learning library for solving differential
  equations.
\newblock \emph{SIAM Review}, 63\penalty0 (1):\penalty0 208--228,
  2021{\natexlab{b}}.
\newblock \doi{10.1137/19M1274067}.

\bibitem[Li et~al.(2021)Li, Zheng, Kovachki, Jin, Chen, Liu, Azizzadenesheli,
  and Anandkumar]{pde_pino_li}
Zongyi Li, Hongkai Zheng, Nikola Kovachki, David Jin, Haoxuan Chen, Burigede
  Liu, Kamyar Azizzadenesheli, and Anima Anandkumar.
\newblock Physics-informed neural operator for learning partial differential
  equations.
\newblock 11 2021.
\newblock \doi{10.48550/arxiv.2111.03794}.
\newblock URL \url{https://arxiv.org/abs/2111.03794v2}.

\bibitem[Wen et~al.(2022)Wen, Li, Azizzadenesheli, Anandkumar, and
  Benson]{fourier_multiphase_wen}
Gege Wen, Zongyi Li, Kamyar Azizzadenesheli, Anima Anandkumar, and Sally~M.
  Benson.
\newblock U-fno—an enhanced fourier neural operator-based deep-learning model
  for multiphase flow.
\newblock \emph{Advances in Water Resources}, 163:\penalty0 104180, 5 2022.
\newblock ISSN 0309-1708.
\newblock \doi{10.1016/J.ADVWATRES.2022.104180}.

\bibitem[You et~al.(2022)You, Zhang, Ross, Lee, and
  Yu]{fno_implicit_materials_you}
Huaiqian You, Quinn Zhang, Colton~J. Ross, Chung-Hao Lee, and Yue Yu.
\newblock Learning deep implicit fourier neural operators (ifnos) with
  applications to heterogeneous material modeling.
\newblock \emph{Computer Methods in Applied Mechanics and Engineering}, 398, 3
  2022.
\newblock \doi{10.1016/j.cma.2022.115296}.
\newblock URL \url{http://arxiv.org/abs/2203.08205
  http://dx.doi.org/10.1016/j.cma.2022.115296}.

\bibitem[Li et~al.(2022{\natexlab{b}})Li, Peng, Yuan, and Wang]{fno_eddy_li}
Zhijie Li, Wenhui Peng, Zelong Yuan, and Jianchun Wang.
\newblock Fourier neural operator approach to large eddy simulation of
  three-dimensional turbulence.
\newblock \emph{Theoretical and Applied Mechanics Letters}, 12:\penalty0
  100389, 11 2022{\natexlab{b}}.
\newblock ISSN 2095-0349.
\newblock \doi{10.1016/J.TAML.2022.100389}.

\bibitem[Bonney et~al.(2022)Bonney, De~Angelis, Dal~Borgo, Andrade, Beregi,
  Jamia, and Wagg]{bonney2022development}
Matthew~S Bonney, Marco De~Angelis, Mattia Dal~Borgo, Luis Andrade, Sandor
  Beregi, Nidhal Jamia, and David~J Wagg.
\newblock Development of a digital twin operational platform using python
  flask.
\newblock \emph{Data-Centric Engineering}, 3, 2022.

\bibitem[Yadav et~al.(2021)Yadav, Agarwal, Gribok, Hays, Pluth, Ritter, Zhang,
  Jain, Ramuhalli, Eskins, et~al.]{yadav2021technical}
Vaibhav Yadav, Vivek Agarwal, Andrei~V Gribok, Ross~D Hays, Adam~J Pluth,
  Christopher~S Ritter, Hongbin Zhang, Prashant~K Jain, Pradeep Ramuhalli, Doug
  Eskins, et~al.
\newblock Technical challenges and gaps in digital-twin-enabling technologies
  for nuclear reactor applications, 2021.

\bibitem[Kobayashi et~al.(2023)Kobayashi, Almutairi, Sakib, Chakraborty, and
  Alam]{kobayashi2023explainable}
Kazuma Kobayashi, Bader Almutairi, Md~Nazmus Sakib, Souvik Chakraborty, and
  Syed~Bahauddin Alam.
\newblock Explainable, interpretable \& trustworthy ai for intelligent digital
  twin: Case study on remaining useful life.
\newblock 2023.

\bibitem[Kumar et~al.(2022{\natexlab{a}})Kumar, Marchi, Alam, Kavka, Koutsawa,
  Rauchs, and Belouettar]{kumar2022multi}
Dinesh Kumar, Mariapia Marchi, Syed~Bahauddin Alam, Carlos Kavka, Yao Koutsawa,
  Gaston Rauchs, and Salim Belouettar.
\newblock Multi-criteria decision making under uncertainties in composite
  materials selection and design.
\newblock \emph{Composite Structures}, 279:\penalty0 114680,
  2022{\natexlab{a}}.

\bibitem[Kumar et~al.(2022{\natexlab{b}})Kumar, Ahmed, Usman, Alajo, and
  Alam]{kumar2022recent}
Dinesh Kumar, Farid Ahmed, Shoaib Usman, Ayodeji Alajo, and Syed Alam.
\newblock Recent advances in uncertainty quantification methods for engineering
  problems.
\newblock \emph{arXiv preprint arXiv:2211.03012}, 2022{\natexlab{b}}.

\bibitem[Kobayashi et~al.(2022{\natexlab{a}})Kobayashi, Bonney, Kumar, and
  Alam]{kobayashi2022practical}
Kazuma Kobayashi, Matthew Bonney, D~Kumar, and Syed Alam.
\newblock Practical applications of gaussian process with uncertainty
  quantification and sensitivity analysis for digital twin for advanced nuclear
  fuel.
\newblock \emph{Handbook of Smart Energy Systems}, 2022{\natexlab{a}}.

\bibitem[Kobayashi et~al.(2022{\natexlab{b}})Kobayashi, Kumar, Bonney,
  Chakraborty, Paaren, and Alam]{kobayashi2022uncertainty}
Kazuma Kobayashi, Dinesh Kumar, Matthew Bonney, Souvik Chakraborty, Kyle
  Paaren, and Syed Alam.
\newblock Uncertainty quantification and sensitivity analysis for digital twin
  enabling technology: Application for bison fuel performance code.
\newblock \emph{Springer Nature Handbook of Smart Energy Systems, arXiv
  preprint arXiv:2210.07541}, 2022{\natexlab{b}}.

\bibitem[Kumar et~al.(2021)Kumar, Alam, Ridwan, and
  Goodwin]{kumar2021quantitative}
Dinesh Kumar, Syed~Bahauddin Alam, Tuhfatur Ridwan, and Cameron~S Goodwin.
\newblock Quantitative risk assessment of a high power density small modular
  reactor (smr) core using uncertainty and sensitivity analyses.
\newblock \emph{Energy}, 227:\penalty0 120400, 2021.

\bibitem[Kobayashi et~al.(2022{\natexlab{c}})Kobayashi, Daniell, Usman, Kumar,
  and Alam]{kobayashi2022surrogate}
Kazuma Kobayashi, James Daniell, Shoaib Usman, Dinesh Kumar, and Syed Alam.
\newblock Surrogate modeling-driven physics-informed multi-fidelity kriging:
  Path forward to digital twin enabling simulation for accident tolerant fuel.
\newblock \emph{Springer Nature Handbook of Smart Energy Systems, arXiv
  preprint arXiv:2210.07164}, 2022{\natexlab{c}}.

\bibitem[Kobayashi et~al.(2022{\natexlab{d}})Kobayashi, Usman, Castano, Alajo,
  Kumar, and Alam]{kobayashi2022data}
Kazuma Kobayashi, Shoaib Usman, Carlos Castano, Ayodeji Alajo, Dinesh Kumar,
  and Syed Alam.
\newblock Data-driven multi-scale modeling and robust optimization of composite
  structure with uncertainty quantification.
\newblock \emph{Springer Nature Handbook of Smart Energy Systems, arXiv
  preprint arXiv:2210.09055}, 2022{\natexlab{d}}.

\bibitem[Kabir(2010{\natexlab{a}})]{kabir2010non}
Hussain Mohammed~Dipu Kabir.
\newblock Non-linear down-sampling and signal reconstruction, without folding.
\newblock In \emph{2010 Fourth UKSim European Symposium on Computer Modeling
  and Simulation}, pages 142--146. IEEE, 2010{\natexlab{a}}.

\bibitem[Kabir(2010{\natexlab{b}})]{kabir2010theory}
Hussain Mohammed~Dipu Kabir.
\newblock A theory of loss-less compression of high quality speech signals with
  comparison.
\newblock In \emph{2010 Fourth UKSim European Symposium on Computer Modeling
  and Simulation}, pages 136--141. IEEE, 2010{\natexlab{b}}.

\bibitem[et~al.(2010{\natexlab{a}})]{kabir2010watermarking}
Hussain Mohammed Dipu~Kabir et~al.
\newblock Watermarking with fast and highly secured encryption for real-time
  speech signals.
\newblock In \emph{2010 IEEE International Conference on Information Theory and
  Information Security}, pages 446--451. IEEE, 2010{\natexlab{a}}.

\bibitem[et~al.(2010{\natexlab{b}})]{kabir2010loss}
Hussain Mohammed Dipu~Kabir et~al.
\newblock A loss-less compression technique for high quality speech signals and
  its implementation with mpeg-4 als for better compression.
\newblock In \emph{2010 IEEE International Conference on Information Theory and
  Information Security}, pages 781--785. IEEE, 2010{\natexlab{b}}.

\bibitem[Garg et~al.(2022{\natexlab{b}})Garg, Chakraborty, and
  Hazra]{garg2022physics}
Shailesh Garg, Souvik Chakraborty, and Budhaditya Hazra.
\newblock Physics-integrated hybrid framework for model form error
  identification in nonlinear dynamical systems.
\newblock \emph{Mechanical Systems and Signal Processing}, 173:\penalty0
  109039, 2022{\natexlab{b}}.

\bibitem[Daniell et~al.(2022)Daniell, Kobayashi, Kumar, Chakraborty, Alajo,
  Taber, Graham, and Alam]{daniell2022physics}
James Daniell, Kazuma Kobayashi, Dinesh Kumar, Souvik Chakraborty, Ayodeji
  Alajo, Ethan Taber, Joseph Graham, and Syed Alam.
\newblock Physics-informed multi-stage deep learning framework development for
  digital twin-centred state-based reactor power prediction.
\newblock \emph{arXiv preprint arXiv:2211.13157}, 2022.

\bibitem[Rahman et~al.(2021)Rahman, Khan, Anowar, Al-Imran, Verma, Kumar,
  Kobayashi, and Alam]{rahman2022leveraging}
M.~Rahman, Abid Khan, Sayeed Anowar, Md~Al-Imran, Richa Verma, Dinesh Kumar,
  Kazuma Kobayashi, and Syed Alam.
\newblock \emph{Leveraging Industry 4.0: Deep Learning, Surrogate Model, and
  Transfer Learning with Uncertainty Quantification Incorporated into Digital
  Twin for Nuclear System}, pages 1--20.
\newblock Springer International Publishing, Cham, 2021.
\newblock ISBN 978-3-030-72322-4.
\newblock \doi{10.1007/978-3-030-72322-4_192-1}.
\newblock URL \url{https://doi.org/10.1007/978-3-030-72322-4_192-1}.

\end{thebibliography}

